Nonlinear stiffness allows passive dynamic hopping for one-legged robots with an upright trunk

Template models are frequently used to simplify the control dynamics for robot hopping or running. Passive limit cycles can emerge for such systems and be exploited for energy-efficient control. A grand challenge in locomotion is trunk stabilization when the hip is offset from the center of mass (CoM). The swing phase plays a major role in this process due to the moment of inertia of the leg; however, many template models ignore the leg mass. In this work, the authors consider a robot hopper model (RHM) with a rigid trunk and leg plus a hip that is displaced from the CoM. It has been previously shown that no passive limit cycle exists for such a model given a linear hip spring. In this work, we show that passive limit cycles can be found when a nonlinear hip spring is used instead. To the authors' knowledge, this is the first time that a passive limit cycle has been found for this type of system.

==> discussion.tex <==
	\section{Discussion}
	
The results of this work demonstrate that a passive dynamic limit cycle may be found for an upright-trunk template model with non-negligible leg mass when a non-linear torsional hip spring stiffness is used. This is in agreement with our first hypothesis. To the authors' knowledge, this is the first time any passive limit cycle has been found for such a system \cite{hyon2004passive}. The results further show that the resulting ground reaction forces intersect at a central point above the center of mass, similar to observations in nature \cite{Maus2010}. This confirms our second hypothesis that the passive limit cycle for the upright trunk model would demonstrate an inherent VPP-GRF-directing behavior. Unsurprisingly, the limit cycle was not stable, as indicated by the $z$ and $\phi$ eigenvalues greater than 1. In agreement with the findings of \cite{hyon2004passive}, we were not able to find a limit cycle for the upright trunk template model when using linear hip spring stiffness (UTLS model).

Base on the work of \cite{hyon2004passive}, the passive limit cycle for the centered-hip linear-spring (CHLS) model was an expected finding. The result that the limit cycle is not passive, with the eigenvalues associated with $z$ and $\theta$ falling outside of the unit circle, was also expected. The passive limit cycle found for the centered-hip nonlinear-spring (CHNS) model was also unstable, but with slightly smaller eigenvalues for all parameters except for $\dot{\phi}$ and the same number of steps to failure (five). Therefore, it can at best be concluded that the nonlinear spring may bring the model slightly closer to a stable limit cycle than the linear-spring version. In both cases, the GRF vectors interested at a point well above the CoM, which may be a necessary condition for a passive limit cycle. This needs to be analyzed further in future research.
%Interestingly, while the limit cycle for the CHLS template model is symmetrical, the upright-trunk exponential-spring (UTES) template model limit cycle demonstrates highly asymmetrical behavior. During the flight phase the hip is rotated into a hyper-extended position before swinging forward to prepare for touchdown. This large angle is needed to generate a sufficiently strong torque in the hip spring in order to reverse the rear rotation of the torso and thus stabilize it during the flight phase.


A necessary condition for complete passive running is that energy is conserved through the gait cycle. In all models' limit cycles, some energy loss was observed, likely corresponding to energy dissipated at touchdown. Based on the equations derived by Hyon and Emura in \cite{hyon2002quasi}, the no energy dissipation condition essentially necessitates that the component of foot velocity that is perpendicular to the leg at touchdown is equal to zero. Given that the forward velocity of the CoM dominates its downward velocity, this is only possible if the leg swing is already in its returning phase at the time of touchdown. This is in agreement with findings in human biomechanics studies \cite{mann1984kinematic}. While reverse leg swing was observed at the point of touchdown for the passive limit cycles of all three systems, it is likely that the necessary condition for no energy dissipation was not achieved, which is supported by initial calculations (results not shown).

Given the passive limit cycle for the upright trunk model, the next step will be to explore stabilization techniques, e.g. local feedback \cite{hyon2004passive}, delayed feedback control \cite{hyon2004energy} or transversal stabilization \cite{manchester2011stable} in order to generate an efficient, stable and robust limit cycle. Toward this aim, other forms of non-linearity should be explored, such as including nonlinear or asymmetrical leg spring stiffness for improved disturbance rejection \cite{karssen2011running,xue2017motion}. Furthermore, better template matching should be considered in a next step, including aspects such as the effect of foot mass and leg retraction as well as the bipedal case.
	
	\section{Conclusion}

Using an exponential torsional spring at the hip, a passive limit cycle was found for an upright-trunk template model, which included non-negligible leg mass, for the first time. This is an important step toward developing simple, energy efficient controllers for inherently unstable robot running and hopping.

==> history/discussion_v1.tex <==
	\section{Discussion}
	
The results of this work demonstrate that a passive dynamic limit cycle may be found for an upright-trunk template model with leg mass when an exponential torsional hip spring stiffness is used. This is in agreement with our first hypothesis. To the authors' knowledge, this is the first time any passive limit cycle has been found for such a system \cite{hyon2004passive}. The results further show that the resulting ground reaction forces intersect at a central point above the center of mass similar to observations in nature \cite{Maus2010}. This confirms our second hypothesis that the system that demonstrates a stable limit cycle would demonstrate an inherent VPP-GRF-directing behavior. 

Base on the work of \cite{hyon2004passive}, the passive limit cycle for the hip-centered linear-spring model was an expected finding. Interestingly, while the limit cycle for the hip-centered linear-spring template model is symmetrical, the upright-trunk nonlinear-spring template model limit cycle demonstrates highly asymmetrical behavior. During the flight phase the hip is strongly hyper-extended before swinging forward to prepare for touchdown. This large angle generates a strong torque at the hip, which is necessary to reverse rear rotation of the torso and thus stabilize it during the flight phase.
	
In agreement with the findings of \cite{hyon2004passive}, we, too, were not able to find a limit cycle for the upright trunk template model when using a linear spring stiffness. An unexpected further result is that we were not able to find a stable limit cycle for the hip-centered model using an exponential spring. It is likely that the required spring characteristics are guided by the morphology of the system. Furthermore, the inherent emergence of VPP-GRF-directing behavior may be a necessary condition for a passive limit cycle, as we also observed this behavior using the hip-centered model with the linear spring. Extended theoretical and computational analysis will be needed to better understand these findings and to apply them to other systems. 

-> Discuss findings from energy plot.

Given the passive limit cycle for the upright trunk model, the next step will be to explore stabilization techniques, e.g. local feedback \cite{hyon2004passive}, delayed feedback control \cite{hyon2004energy} or transversal stabilization \cite{manchester2011stable} in order to generate an efficient, stable and robust limit cycle. Toward this aim, other forms of non-linearity should be explored, such as including nonlinear or asymmetrical leg spring stiffness for improved disturbance rejection \cite{karssen2011running,xue2017motion}. Furthermore, better template matching should be considered in a next step, including aspects such as the effect of foot mass and leg retraction as well as the bipedal case.
	
	\section{Conclusion}

Using an exponential torsional spring at the hip, a passive limit cycle was found for an upright-trunk template model for the first time. This is an important step toward developing simple, energy efficient controllers for inherently unstable robot running and hopping.

==> history/discussion_v2.tex <==
	\section{Discussion}
	
The results of this work demonstrate that a passive dynamic limit cycle may be found for an upright-trunk template model with leg mass when an exponential torsional hip spring stiffness is used. This is in agreement with our first hypothesis. To the authors' knowledge, this is the first time any passive limit cycle has been found for such a system \cite{hyon2004passive}. The results further show that the resulting ground reaction forces intersect at a central point above the center of mass similar to observations in nature \cite{Maus2010}. This confirms our second hypothesis that the system and initial conditions that produce a stable limit cycle would also demonstrate an inherent VPP-GRF-directing behavior. 

Base on the work of \cite{hyon2004passive}, the passive limit cycle for the hip-centered linear-spring model was an expected finding. Interestingly, while the limit cycle for the hip-centered linear-spring template model is symmetrical, the upright-trunk exponential-spring template model limit cycle demonstrates highly asymmetrical behavior. During the flight phase the hip is rotated into a hyper-extended position before swinging forward to prepare for touchdown. This large angle is needed to generate a sufficiently strong torque in the hip spring in order to reverse the rear rotation of the torso and thus stabilize it during the flight phase.
	
In agreement with the findings of \cite{hyon2004passive}, we were not able to find a limit cycle for the upright trunk template model when using linear spring stiffness. %Need to confirm this!!!%
An unexpected further result is that we were not able to find a stable limit cycle for the hip-centered model using an exponential spring. It is likely that the required spring characteristics are guided by the morphology and innate stability attributes of the system. Furthermore, the inherent emergence of VPP-GRF-directing behavior may be a necessary condition for a passive limit cycle, as we also observed this behavior using the hip-centered model with the linear spring. %Potentially add: In fact, neither the upright-trunk linear-spring nor the hip-centered exponential-spring systems, for which no stable limit cycle was found, demonstrate VPP-GRF-directing behavior.
Extended theoretical and computational analysis will be needed to better understand these findings and to apply them to other systems. 

A necessary condition for complete passive running is that energy is conserved through the gait cycle. For the current systems, this means that no energy may be dissipated at touchdown. Based on the equations derived by Hyon and Emura in \cite{hyon2002quasi}, the no energy dissipation condition essentially necessitates that the component of foot velocity that is perpendicular to the leg at touchdown is equal to zero. Given that the forward velocity of the CoM dominates its downward vertical velocity, this is only possible if the leg swing is already in its returning phase at the time of touchdown. %Consider referring to biomechanics literature here.%
Based on the energy plots, there is visible energy loss over the passive limit cycle of the upright-trunk system but not of the hip-centered system. We also see for the hip-centered system that the hip swing is returning at the time of ground impact, which is possible due to the symmetrical nature of the limit cycle.  %Show plot for this?%
This is in contrast to the asymmetrical nature of the upright-torso system limit cycle, where the hip is still in the forward swing phase at the time of impact. Therefore, the necessary condition of energy conservation at impact is not met for the upright-trunk system. The resulting energy dissipation at touchdown likely explains, at least in part, why the upright-trunk system achieves fewer steps before falling than the hip-centered system.

Given the passive limit cycle for the upright trunk model, the next step will be to explore stabilization techniques, e.g. local feedback \cite{hyon2004passive}, delayed feedback control \cite{hyon2004energy} or transversal stabilization \cite{manchester2011stable} in order to generate an efficient, stable and robust limit cycle. Toward this aim, other forms of non-linearity should be explored, such as including nonlinear or asymmetrical leg spring stiffness for improved disturbance rejection \cite{karssen2011running,xue2017motion}. Furthermore, better template matching should be considered in a next step, including aspects such as the effect of foot mass and leg retraction as well as the bipedal case.
	
	\section{Conclusion}

Using an exponential torsional spring at the hip, a passive limit cycle was found for an upright-trunk template model for the first time. This is an important step toward developing simple, energy efficient controllers for inherently unstable robot running and hopping.

==> history/intro_v1.tex <==

	\section{Introduction}
Running, or hopping, is a highly dynamic process of an inherently unstable system and it remains a mystery to this day how humans and animals are able to accomplish such a complex task with high efficiency and minimal concentration (i.e. computational complexity). There are a number of strategies being pursued in an attempt to achieve similar feats in robotic locomotion. Reduced order and compliant control approaches, for example using template models, are one area that are explored extensively toward this aim \cite{ahmadi1997stable}.  \\

Blickhan's spring-loaded inverted pendulum (SLIP; \cite{Blickhan89}) and its variants remain some of the most heavily used template models for robot control. However, because the legs are considered massless in typical SLIP models, the swing phase dynamics are ignored and the swing function is limited to optimally setting the angle of attack for stable landing \cite{Blum2010,Raibert86}. Thus, important locomotion challenges associated with e.g. torso stabilization, synchronization of hip swing with vertical motion and touchdown angle requirements, as well as passive dynamics matching are ignored in these models. One noteable exception is a template model that is made up of a rigid torso and leg with non-neglible mass and moment of inertia as well as a hip and (lower) leg spring \cite{thompson1990passive}. This model represents the full body dynamics (including the physical interaction between the legs and the torso) during both the stance and swing phases of gait. This model can be further extended to represent an upright torso by displacing the hip from the center of mass (COM), as shown in \cite{hyon2004passive}. \\

One of the many benefits of a template model is the ability to explore passive dynamic limit cycles. Minimizing energy requirement (or metabolic cost) is a strong motivation in robotics \cite{ahmadi1997stable} and is a fundamental principle behind animal locomotion \cite{sasaki2006muscle}. Moreover, biological locomotion is characterized by high dexterity and robustness with presumably low computational complexity, as demonstrated by the relatively low signal frequency, low control bandwidth, and high signal delay of humans vs. robots \cite{Winter1998}. Thompson and Raibert showed that fully passive (dynamic running could be achieved using a SLIP model, given the necessary input conditions; though the resulting limit cycle is not stable \cite{thompson1990passive}. Since then it has been shown that, given a passive limit cycle, active stabilization and disturbance rejection can be achieved using relatively simple controllers while exploiting the energy savings of the passive dynamics \cite{ahmadi1997stable, hyon2004passive, hyon2004energy}. However, this approach has not yet been successfully applied to an upright trunk model because no passive limit cycle could be found \cite{hyon2004passive}. \\

In recent biomechanics literature \cite{Maus2010} it has been shown that an indirect trunk stabilization strategy can be observed in humans and animals. During stance, the ground reaction forces (GRFs) intersect at a point above the CoM. This has the effect that the CoM behaves like it is hanging from the intersection point - forming a virtual pendulum and indirectly stabilizing the upper body. The intersection point is sometimes also called the virtual pivot point (VPP).
Sharbafi et al \cite{Sharbafi2012} approached this empirical finding by developing a VPP-based controller for trunk stabilization. However, it is unlikely that the trajectory of the ground reaction force with respect to the dynamic VPP could be adequately represented by a biological nervous system to be used as a control target; thus, this empirical observation more likely points to another regulatory mechanism out of which the VPP-GRF-directing behavior emerges \cite{gruben2012force}. Identifying this regulatory mechanism could be the key to finding a passive limit cycle for the unified stance-swing template model with upright trunk. \\

We hypothesize that a passive dynamic limit cycle may be found for an upright trunk model by using a non-linear (exponential) torsional hip spring. Furthermore, we hypothesize that this passive limit cycle will demonstrate an inherent VPP-GRF-directing behavior of the system. \\



==> history/intro_v2.tex <==
\section{Introduction}
Running, or hopping, is a highly dynamic process of an inherently unstable system and it remains a mystery to this day how humans and animals are able to accomplish such a complex task with high efficiency and minimal concentration (i.e. computational complexity). There are a number of strategies being pursued in an attempt to achieve similar feats in robotic locomotion. Reduced order and compliant control approaches, for example using template models, are one area that are explored extensively toward this aim \cite{ahmadi1997stable}.  

Blickhan's spring-loaded inverted pendulum (SLIP; \cite{Blickhan89}) and its variants remain some of the most heavily used template models for robot control. However, because the legs are considered massless in typical SLIP models, the swing phase dynamics are ignored and the swing function is limited to optimally setting the angle of attack for stable landing \cite{Blum2010,Raibert86}. Thus, important locomotion challenges associated with e.g. torso stabilization, synchronization of hip swing with vertical motion and touchdown angle requirements, as well as passive dynamics matching are ignored in these models. One noteable exception is a robot hopping template model (RHM) that is made up of a rigid trunk and leg with non-neglible moment of inertia as well as a hip and (lower) leg spring \cite{thompson1990passive}. This model represents the full body dynamics (including the physical interaction between the legs and the torso) during both the stance and swing phases of gait. This model can be further extended to represent an upright torso by displacing the hip from the center of mass (CoM), as shown in \cite{hyon2004passive}. 

One of the many benefits of a template model is the ability to explore passive dynamic limit cycles. Minimizing energy requirement (or metabolic cost) is a strong motivation in robotics \cite{ahmadi1997stable} and is a fundamental principle behind animal locomotion \cite{sasaki2006muscle}. Moreover, biological locomotion is characterized by high dexterity and robustness with presumably low computational complexity, as demonstrated by the relatively low signal frequency, low control bandwidth, and high signal delay of humans vs. robots \cite{Winter1998}. Thompson and Raibert showed that, given the necessary input conditions, fully passive dynamic running could be achieved using their RHM model with the hip located at the trunk CoM \cite{thompson1990passive}. However, the resulting limit cycle is not stable. A purely passive locomotion approach is not realistic for mechanical systems, of course, because of unavoidable mechanical losses. Rather, the idea is to tune the gait of the target robotic system using this approach, so that the passive energy return, and thus efficiency, is optimized. In fact, it has been shown that, given a passive limit cycle, active stabilization and disturbance rejection can be achieved using relatively simple controllers while exploiting the energy savings of the passive dynamics \cite{ahmadi1997stable, hyon2004passive, hyon2004energy}. However, this approach has not yet been successfully applied to an upright trunk model because no passive limit cycle could be found \cite{hyon2004passive}. 

In recent biomechanics literature \cite{Maus2010} it has been shown that an indirect trunk stabilization strategy can be observed in humans and animals. During stance, the ground reaction forces (GRFs) intersect at a point above the CoM. This has the effect that the CoM behaves like it is hanging from the intersection point - forming a virtual pendulum and indirectly stabilizing the upper body. The intersection point is sometimes also called the virtual pivot point (VPP).
Sharbafi et al \cite{Sharbafi2012} approached this empirical finding by developing a VPP-based controller for trunk stabilization. However, it is unlikely that the trajectory of the ground reaction force with respect to the dynamic VPP could be adequately represented by a biological nervous system to be used as a control target; thus, this empirical observation more likely points to another regulatory mechanism out of which the VPP-GRF-directing behavior emerges \cite{gruben2012force}. Identifying this regulatory mechanism could be the key to finding a passive limit cycle for the unified stance-swing template model with upright trunk. 

We hypothesize that a passive dynamic limit cycle may be found for an upright trunk model with a non-negligible leg moment of inertia by using a non-linear (cubic) torsional hip spring (referred to as the upright-trunk nonlinear-spring, UTNS, model). We further hypothesize that this passive limit cycle will demonstrate an inherent VPP-GRF-directing behavior of the system. Finally, as a means of comparison we investigated whether a similar non-linear hip spring may be used to increase the stability of the same model with the hip centered at the CoM (i.e. centered-hip nonlinear-spring, CHNL, model).



==> results.tex <==
\section{Results}
A passive limit cycle was found for the centered-hip linear-spring (CHLS) model described by \cite{hyon2004passive} with identical parameters (see Table \ref{tbl:values}) and a fixed forward velocity of $\dot{x}= 5 \frac{\mathrm{m}}{\mathrm{s}}$. The fixed point and the eigenvalues of the monodromy matrix can be found in Tables \ref{tbl:fixpt} and \ref{tbl:eig}. As can be seen, the eigenvalues of parameters $z$ and ${\theta}$ are $-5.775$ and $2.243$, respectively, indicating that the found limit cycle is not stable. The simulation was able to complete 5 steps before failure. The change in kinetic energy over the gait cycle was found to be $-0.012$$J$. A visualization of this gait can be seen in Fig. \ref{fig:Hyon} and the associated GRF vectors can be viewed in Fig. \ref{fig:GRF}.




\begin{table}
	\centering
	%\label{tbl:fixpt}	
	%Table II \quad Fixed points for centered-hip linear-spring (CHLS), centered-hip nonlinear-spring (CHNS) and upright-trunk nonlinear-spring (UTNS) models. The values correspond to the state vector, \mbox{$\vect{x} = \left[x, z, \theta, \phi, l\right, \dot{x}, \dot{z}, \dot{\theta}, \dot{\phi}, \dot{l\right}]^{\mathsf{T}}$}. \vspace{0.25cm}
	\caption{Fixed points for centered-hip linear-spring (CHLS), centered-hip nonlinear-spring (CHNS) and upright-trunk nonlinear-spring (UTNS) models. The values correspond to the state vector, $\vect{x} = [x, z, \theta, \phi, l, \dot{x}, \dot{z}, \dot{\theta}, \dot{\phi}, \dot{l}]^{\mathsf{T}}$.} \label{tbl:fixpt}
	\begin{tabularx}{0.4\textwidth}{c|c|c}
		HCLS & HCNS & UTNS \\
		\hline
		& & \\
		$ \begin{bmatrix} 0.000 \\
		0.6371\\
		9.905e-08\\
		-1.119e-07\\
		0.5000\\
		5.000\\
		0.0000\\
		-1.780\\
		10.45\\
		0.000
		\end{bmatrix} $  & $ \begin{bmatrix}
		0.000\\
		0.5793\\
		1.752e-06\\
		-8.053e-07\\
		0.5000\\
		5.000\\
		0.000\\
		-1.589\\
		9.445\\
		0.000 \end{bmatrix} $ & $ \begin{bmatrix}
		0.000\\
		1.000\\
		6.459e-06\\
		5.892e-06\\
		0.5000\\
		5.000\\
		0.000\\
		-0.5869\\
		6.836\\
		0.000 \end{bmatrix} $      
	\end{tabularx}		
\end{table}



\begin{table}
	\centering
	%\label{tbl:eig}	
	%Table III \quad Eigenvalues for centered-hip (top) and upright-trunk (bottom) models with linear (left) and nonlinear (right) springs. The variables correspond to the reduced state vector, $\vect{x}_{red} = [z, \theta, \phi, \dot{x}, \dot{\theta}$. \vspace{0.25cm}
	\caption{Eigenvalues for centered-hip (top) and upright-trunk (bottom) models with linear (left) and nonlinear (right) springs. The variables correspond to the reduced state vector, $\vect{x}_{red} = [z, \theta, \phi, \dot{x}, \dot{\theta}]$.} \label{tbl:eig}
	\begin{tabularx}{0.4\textwidth}{l|c|c}
		& Linear spring & Nonlinear spring\\
		\hline
		& & \\
		\multirow{3}{1.0cm}{Centered-hip model} & $ \begin{bmatrix} (-5.775,0) \\
		2.243\\
		1.000/\
		-0.1868\\
		-0.05112\\
		-1.234e-05\\
		\end{bmatrix}$ &$ \begin{bmatrix}
		-3.475\\
		1.621\\
		1.000\\
		0.04849\\
		3.021e-06\\
		-0.7732 \end{bmatrix}$ \\
		& & \\
		\hline
		& & \\
		\multirow{3}{1.2cm}{Upright-trunk model} & $-$ & $\begin{bmatrix}
		33.51\\
		0.4894 -0.9437i\\
		-9.422\\
		0.9995\\
		0.1172\\
		0.01830\\
		-0.0003156\\
		\end{bmatrix}$   
	\end{tabularx}		
\end{table}


\begin{figure}
	\vspace{-3cm}
	\import{./python/}{GRF_neu.pgf}
	\caption{Normalized ground reaction force vectors in the CoM frame of reference for the CHLS (top), CHNS (middle) and UTNS (bottom) models. In all cases the vectors are directed well above the CoM.}\label{fig:GRF}
\end{figure}



\begin{figure*} 
	\includegraphics[width=0.33\textwidth]{./pics/Hyon/1.png}
	\includegraphics[width=0.33\textwidth]{./pics/Hyon/2.png}
	\includegraphics[width=0.33\textwidth]{./pics/Hyon/3.png}
	\includegraphics[width=0.33\textwidth]{./pics/Hyon/4.png}
	\includegraphics[width=0.33\textwidth]{./pics/Hyon/5.png}
	\includegraphics[width=0.33\textwidth]{./pics/Hyon/6.png}
	\caption{Visualization of limit cycle jumping for the centered-hip nonlinear-spring model. The images were rendered with the open-source software MeshUp (https://github.com/ORB-HD/MeshUp).}\label{fig:Hyon}
\end{figure*}


	\begin{figure*} 
	\includegraphics[width=0.33\textwidth]{./pics/Hip/1.png}
	\includegraphics[width=0.33\textwidth]{./pics/Hip/2.png}
	\includegraphics[width=0.33\textwidth]{./pics/Hip/3.png}
	\includegraphics[width=0.33\textwidth]{./pics/Hip/4.png}
	\includegraphics[width=0.33\textwidth]{./pics/Hip/5.png}
	\includegraphics[width=0.33\textwidth]{./pics/Hip/6.png}
	\caption{Visualization of limit cycle jumping for the upright-trunk nonlinear-spring model. The images were rendered with the open-source software MeshUp (https://github.com/ORB-HD/MeshUp).} \label{fig:Hip}
\end{figure*}


The search for a passive limit cycle for the upright-trunk linear-spring (UTLS) model was unsucessful. However, the remaining two variations on the model described by \cite{hyon2004passive} also yielded passive limit cycles: the centered-hip nonlinear-spring (CHNS) and the upright-trunk nonlinear-spring (UTNS) model. In each case, the same model parameters and fixed velocity were used as in the first case with the exception of the hip location for the UTLS and UTNS models, which were displaced by a factor of $d$. The fixed points and the eigenvalues of the monodromy matrix can again be found in Tables \ref{tbl:fixpt} and \ref{tbl:eig}. Both limit cycles are unstable, indicated by the eigenvalues greater than 1. The $z$ and ${\theta}$ parameters of the CHNS model have eigenvalues of $-3.475$ and $1.621$, respectively, while the $z$ and ${\phi}$ parameters of the UTNS model have eigenvalues of $33.51$ and$ -9.422$, respectively. Accordingly, the CHNS model simulation reached 5 steps before failure and the UTNS model reached 3 steps before failure. The energy loss over the gait cycle was found to be $-0.002$$J$ and $-0.016$$J$, respectively. The GRF vectors of both simulations can be viewed in Fig. \ref{fig:GRF}. The limit cycle of the UTNS model is depicted in Fig. \ref{fig:phase} and a visualization of the corresponding gait can be seen in Fig. \ref{fig:Hip}.
